Instructions and Guide for Diagnostic Questions: The NeurIPS 2020 Education Challenge

Digital technologies are becoming increasingly prevalent in education, enabling personalized, high quality education resources to be accessible by students across the world. Importantly, among these resources are diagnostic questions: the answers that the students give to these questions reveal key information about the specific nature of misconceptions that the students may hold. Analyzing the massive quantities of data stemming from students' interactions with these diagnostic questions can help us more accurately understand the students' learning status and thus allow us to automate learning curriculum recommendations. In this competition, participants will focus on the students' answer records to these multiple-choice diagnostic questions, with the aim of 1) accurately predicting which answers the students provide; 2) accurately predicting which questions have high quality; and 3) determining a personalized sequence of questions for each student that best predicts the student's answers. These tasks closely mimic the goals of a real-world educational platform and are highly representative of the educational challenges faced today. We provide over 20 million examples of students' answers to mathematics questions from Eedi, a leading educational platform which thousands of students interact with daily around the globe. Participants to this competition have a chance to make a lasting, real-world impact on the quality of personalized education for millions of students across the world.

==> metrics.tex <==

\iffalse
\section{Metrics}

The metrics for each task are as follows:
\begin{enumerate}
    \item \textbf{Task 1:} Prediction accuracy $A$ -- the number of predictions that match the true correctness indicator, divided by the total number of predictions (in the held-out test set): 
    $A = \frac{N_{correct\_predictions}}{N_{total\_predictions}}$.
    
    \item \textbf{Task 2:} Prediction accuracy as above, except that the true answers are now categorical instead of binary.
    
    \item \textbf{Task 3:} The participants will submit a quality ranking for the questions (Figure \ref{fig:task3metric} \textit{Left}). An unseen set of question-pairs will then be used to evaluate the quality of this ranking (and thus the underlying metric). Note that we have collected the experts' judgement of which question in each pair is of higher quality. The evaluation steps are then as follows (see also Figure \ref{fig:task3metric} \textit{Right} for an illustration):
    \begin{itemize}
        \item Determine, based on the submitted ranking, which question in each pair is of higher quality.
        \item Compare this with each expert's judgement (assign 1 if matching, 0 if not matching).
        \item For each expert $i$, determine the agreement fraction: $A_i = \frac{N_{matching\_pairs}}{N_{total\_pairs}}$ .
        \item Find the \textit{maximum} of these agreement fractions $A_{max} = \max_{i} A_i$. This will be used as the final evaluation metric for this task.
    \end{itemize}
    
    We are using looking for metrics that can approximate \textit{an} expert judgement really well, hence we use the maximum of the agreement fractions, rather than a mean of the agreement fractions over all experts. The reasoning for this approach is that the quality metrics of the experts are in themselves subjective, and it is interesting to find whether a particular expert's approach can be approximated especially well by the use of machine learning. \al{Double check we are actually reporting the mean afterwards} Note that we will report the mean of the agreement fractions metric at the end of the competition, but this will not be used to judge the task winner.

    \item \textbf{Task 4: } Submitted models will be asked to sequentially choose 10 query questions for each student in a held-out set of students, with the answer to each question revealed to the model in private after selection. The model is given the opportunity to incorporate this information or retrain after each question. After receiving 10 answers for each student, the model will be assessed on its prediction accuracy on a held-out test set of answers for each of these students, that cannot be queried. \al{current scoring setup just uses binary data} As in Task 1, binary data will be used for this task.

%\[\textrm{MRR} = \frac{1}{|\mathcal{S}|}\sum_{i=1}^{|\mathcal{S}|}\frac{1}{\textrm{rank}_i}\]
\end{enumerate}

\fi

==> rules.tex <==
% \section{Rules}
% \CZ{We can put this to the last section. They are much less important than the getting started section}
% \al{Need to review these, they're old}

% \noindent

% The rules of the competition are as follows: 
% \begin{itemize}
% \item Users may work in teams of up to 10 people. 
% \item In tasks that require a code submission to be executed, entrant's code must run on the provided compute environment within 1 hour. This is to encourage computationally efficient solutions appropriate for real-time personalized education.
% \item During the evaluation of the submitted code, the individual containers will not have access to any external network to avoid any information leak.
% \item The submitted code must generate predictions using a machine learning model. Submissions making hard-coded predictions are forbidden.
% \item Users may make use of open source libraries given proper attribution. At the end of the competition, we encourage all code to be open-sourced so the results can be reproduced. 
% \item The use of supplementary existing open-source datasets for e.g. pre-training is permitted provided they are credited. The use of private, proprietary datasets is not permitted.
% \item The questions images have been shared solely for the purpose of this competition and must not be used for any other purpose. The question images must not printed or shared with anyone outside of the competition.
% \item Any parties or individuals affiliated with Eedi, Microsoft Research or the Computational and Biological Learning Group, University of Cambridge are not eligible for the prizes, but may participate in the competition.
% \item For participants to be eligible for prizes their code must be publicly available. 
% \item Any instances of cheating, defined as violation of the rules above or any other attempt to circumvent the spirit and intent of the competition, as determined by the organizers, will result in the invalidation of all of the offending team's submissions and a disqualification from the competition.
% \end{itemize}


% In order to prevent cheating, all the evaluation data will be kept completely inaccessible to the participants during the competition. The aforementioned rules on manual review of the submissions and lack of network access during code evaluation also aim to prevent cheating.
